UNIP: Rethinking Pre-trained Attention Patterns for Infrared Semantic Segmentation

Pre-training techniques significantly enhance the performance of semantic segmentation tasks with limited training data. However, the efficacy under a large domain gap between pre-training (e.g. RGB) and fine-tuning (e.g. infrared) remains underexplored. In this study, we first benchmark the infrared semantic segmentation performance of various pre-training methods and reveal several phenomena distinct from the RGB domain. Next, our layerwise analysis of pre-trained attention maps uncovers that: (1) There are three typical attention patterns (local, hybrid, and global); (2) Pre-training tasks notably influence the pattern distribution across layers; (3) The hybrid pattern is crucial for semantic segmentation as it attends to both nearby and foreground elements; (4) The texture bias impedes model generalization in infrared tasks. Building on these insights, we propose UNIP, a UNified Infrared Pre-training framework, to enhance the pre-trained model performance. This framework uses the hybrid-attention distillation NMI-HAD as the pre-training target, a large-scale mixed dataset InfMix for pre-training, and a last-layer feature pyramid network LL-FPN for fine-tuning. Experimental results show that UNIP outperforms various pre-training methods by up to 13.5\% in average mIoU on three infrared segmentation tasks, evaluated using fine-tuning and linear probing metrics. UNIP-S achieves performance on par with MAE-L while requiring only 1/10 of the computational cost. Furthermore, UNIP significantly surpasses state-of-the-art (SOTA) infrared or RGB segmentation methods and demonstrates broad potential for application in other modalities, such as RGB and depth. Our code is available at https://github.com/casiatao/UNIP.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tab_tex/attn_vs_feat.tex <==
\begin{table}[t]
    \centering
    \caption{Ablations for distillation targets. The teacher and student models are MAE-L and UNIP-S.}
    \label{tab:target_ablation}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.2mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c}
        \toprule
        Target & Layer & SODA & MFNet-T & SCUT-Seg & Mean \\
        \midrule
        \multirow{2}{*}{Feature} & 18 & 66.03 & 48.83 & 66.06 & 60.31  \\
        & 24 & 66.41 & 49.56 & 67.28 & 61.08  \\
        \midrule
        \multirow{2}{*}{Attention} & \rowcolor{cyan!15} 18 & \textbf{70.99} & \textbf{51.32} & \textbf{70.79} & \textbf{64.37}  \\
        & 24 & 67.74 & 50.39 & 69.00 & 62.38  \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/correlation_coeff.tex <==
\begin{table}[t]
  \begin{minipage}{0.49\linewidth}
    \caption{Correlation coefficients between the average fine-tuning performance and other metrics.}
    \label{tab:correlation_coeff}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{0.8mm}{
    \scalebox{0.95}{
    \begin{tabular}{c c c c c c}
        \toprule
        Performance Metric & Correlation metric & Small & Base & Large & Mean \\
        \midrule
        \multirow{2}{*}{Linear probe} & Pearson & 0.89 & 0.93 & 0.89 & 0.90  \\
        & Spearman & 1.00 & 1.00 & 1.00 & 1.00 \\
        \midrule
        \multirow{2}{*}{ImageNet Acc} & Pearson & 0.78 & 0.12 & -0.90 & 0.00 \\
        & Spearman & 0.83 & 0.64 & -1.00 & 0.16 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
    \end{minipage}
  \hfill
  \begin{minipage}{0.49\linewidth}
  \caption{The LLP performance on RGB datasets. Training epochs are 30 and 100 for ADE20K and MFNet-RGB.}
    \label{tab:rgb_llp}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{0.9mm}{
    \scalebox{0.95}{
    \begin{tabular}{c c c c c c}
        \toprule
        \multirow{2}{*}{Datasets} & \multicolumn{2}{c}{DINO-Small} & \multicolumn{2}{c}{DeiT-Small} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & Layer 9 & Layer 12 & Layer 9 & Layer 12 \\
        \midrule
        ADE20K \citep{ade20k} & \textbf{26.11} & 23.15 & \textbf{24.35} & 22.68  \\
        MFNet-RGB \citep{mfnet} & \textbf{38.94} & 37.53  & \textbf{30.43} & 29.44 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
  \end{minipage}
\end{table}

==> tab_tex/data_and_fpn.tex <==
\begin{table}[t]
  \begin{minipage}{0.52\linewidth}
  \centering
    \caption{Ablations for components of the InfMix dataset. The teacher and student models are MAE-L and UNIP-S. All datasets are distilled for the same number of iterations to ensure a fair comparison.}
    \label{tab:dataset_composition_ablation}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.0mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c}
        \toprule
        Dataset & \#Images & SODA & MFNet-T & SCUT-Seg & Mean \\
        \midrule
        \rowcolor{cyan!15} InfMix & 859,375 & \textbf{70.99} & \textbf{51.32} & 70.79 & \textbf{64.37} \\
        -- w/o IN1K 200K & 659,375 & 69.41 & 51.13 & 70.21 & 63.58 \\
        -- w/o COCO & 741,088 & 69.62 & 51.29 & 69.58 & 63.50 \\
        -- w/o Grayscale & 859,375 & 69.73 & 50.71 & \textbf{71.09} & 63.84 \\
        \midrule
        ImageNet-1K & 1,281,167 & 69.39	& 49.11 & 69.63 & 62.71 \\ 
        InfPre & 541,088 & 68.45 & 51.27 & 67.87 & 62.53 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
  \end{minipage}
  \hfill
  \begin{minipage}{0.47\linewidth}
    \centering
    \caption{Ablations for the LL-FPN. \xmark\, and \cmark\, denote the ones in \figref{fig:ft_lp}\textcolor{red}{a} and \figref{fig:ft_lp}\textcolor{red}{c}. The student models are UNIP-S.}
    \label{tab:fpn_ablation}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.0mm}{
    \scalebox{0.97}{
    \begin{tabular}{l c c c c c}
        \toprule
        Teacher & LL-FPN & SODA & MFNet-T & SCUT-Seg & Mean \\
        \midrule
        \multirow{2}{*}{\makecell[c]{MAE-L \\ (Layer 18)}} & \xmark & 69.54 & 50.18 & 70.63 & 63.45 \\
        & \cellcolor{cyan!15}\cmark & \cellcolor{cyan!15}\textbf{70.99} & \cellcolor{cyan!15}\textbf{51.32} & \cellcolor{cyan!15}\textbf{70.79} & \cellcolor{cyan!15}\textbf{64.37} \\
        \midrule
        \multirow{2}{*}{\makecell[c]{MAE-L \\ (Layer 24)}} & \xmark & 69.54 & 50.18 & 70.63 & 63.45 \\
        & \cellcolor{cyan!15}\cmark & \cellcolor{cyan!15}\textbf{70.99} & \cellcolor{cyan!15}\textbf{51.32} & \cellcolor{cyan!15}\textbf{70.79} & \cellcolor{cyan!15}\textbf{64.37} \\
        \midrule
        \multirow{2}{*}{\makecell[c]{DINO-B \\ (Layer 9)}} & \xmark & 68.56 & 49.44 & 68.49 & 62.16 \\
        & \cellcolor{cyan!15}\cmark & \cellcolor{cyan!15}\textbf{69.35} & \cellcolor{cyan!15}\textbf{49.95} & \cellcolor{cyan!15}\textbf{69.70} & \cellcolor{cyan!15}\textbf{63.00} \\
        \midrule
        \multirow{2}{*}{\makecell[c]{DINO-B \\ (Layer 12)}} & \xmark & 68.56 & 49.44 & 68.49 & 62.16 \\
        & \cellcolor{cyan!15}\cmark & \cellcolor{cyan!15}\textbf{69.35} & \cellcolor{cyan!15}\textbf{49.95} & \cellcolor{cyan!15}\textbf{69.70} & \cellcolor{cyan!15}\textbf{63.00} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
  \end{minipage}
\end{table}

==> tab_tex/data_ratio.tex <==
\begin{table}[t]
    \caption{The FT performance of using different sizes of InfMix as the pre-training dataset. The images are evenly sampled from each sub-dataset. The teacher and student models are MAE-L and UNIP-S.}
    \label{tab:data_ratio}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.0mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c}
        \toprule
        Ratio & \#Images & SODA & MFNet-T & SCUT-Seg & Mean \\
        \midrule
        1\% & 8,594 & 20.61 & 16.10 & 31.24 & 22.65 \\
        10\% & 85,938 & 59.66 & 38.80 & 57.72 & 52.06 \\
        30\% & 257,813 & 68.29 & 50.39 & 69.04 & 62.57  \\
        \rowcolor{cyan!15} 100\% & 859,375 & \textbf{70.99} & \textbf{51.32} & \textbf{70.79} & \textbf{64.37} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/dataset_composition_ablation.tex <==
\begin{table}[t]
    \centering
    \caption{Ablations for components of the mixed dataset. The teacher and student models are MAE-L and UNIP-S, respectively.}
    \label{tab:dataset_composition_ablation}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.2mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c}
        \toprule
        Dataset & \#Images & SODA & MFNet-T & SCUT-Seg & Mean \\
        \midrule
        ImageNet-1K & 1,281,167 & 69.39	& 50.41 & 69.63 & 63.14 \\ 
        \midrule
        \rowcolor{cyan!15} Mixed Dataset & 859,375 & \textbf{70.99} & \textbf{51.32} & 70.79 & \textbf{64.37} \\
        -- w/o IN1K 200K & 659,375 & 69.41 & 51.13 & 70.21 & 63.58 \\
        -- w/o COCO & 741,088 & 69.62 & 51.29 & 69.58 & 63.50 \\
        -- w/o Grayscale & 859,375 & 69.73 & 50.71 & \textbf{71.09} & 63.84 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/distill_and_sota.tex <==
\begin{table}[t]
  \begin{minipage}{0.47\linewidth}
  \centering
    \caption{FT performance of different models.}
    \label{tab:main_distill}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{0.8mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c}
        \toprule
        Methods & Params(M) & SODA & MFNet-T & SCUT-Seg & Mean \\
        \midrule
        \textcolor{gray}{MAE-L} & \textcolor{gray}{441.3} & \textcolor{gray}{71.04} & \textcolor{gray}{51.17} & \textcolor{gray}{70.83} & \textcolor{gray}{64.35} \\
        MAE-T & 11.0 & 52.85 & 35.93 & 51.31 & 46.70 \\
        \rowcolor{cyan!15} UNIP-T & 11.0 & \textbf{64.83} & \textbf{48.77} & \textbf{67.22} & \textbf{60.27} \\
        & & \plus{+11.98} & \plus{+12.84} & \plus{+15.91} & \plus{+13.57} \\
        % \cmidrule(lr){1-6}
        MAE-S & 41.9 & 63.36 & 42.44 & 60.38 & 55.39 \\
        \rowcolor{cyan!15} UNIP-S & 41.9 & \textbf{70.99} & \textbf{51.32} & \textbf{70.79} & \textbf{64.37}  \\
        & & \plus{+7.63} & \plus{+8.88} & \plus{+10.41} & \plus{+8.98} \\
        MAE-B & 163.7 & 68.18 & 46.78 & 67.86 & 60.94 \\
        \rowcolor{cyan!15} UNIP-B & 163.7 & \textbf{71.47} & \textbf{52.55} & \textbf{71.82} & \textbf{65.28} \\
        & & \plus{++3.29} & \plus{+5.77} & \plus{+3.96} & \plus{+4.34} \\
        \midrule
        \textcolor{gray}{DINO-B} & \textcolor{gray}{163.7} & \textcolor{gray}{69.79} & \textcolor{gray}{48.54} & \textcolor{gray}{69.82} & \textcolor{gray}{62.72} \\
        DINO-S & 41.9 & 68.56 & 47.98 & 68.74 & 61.76 \\
        \rowcolor{cyan!15} UNIP-S & 41.9 & \textbf{69.35} & \textbf{49.95} & \textbf{69.70} & \textbf{63.00} \\
        & & \plus{+0.79} & \plus{+1.97} & \plus{+0.96} & \plus{+1.24} \\
        \midrule
        \textcolor{gray}{iBOT-L} & \textcolor{gray}{441.3} & \textcolor{gray}{71.75} & \textcolor{gray}{51.66} & \textcolor{gray}{71.49} & \textcolor{gray}{64.97} \\
        iBOT-S & 41.9 & 69.33 & 47.15 & 69.80 & 62.09 \\
        \rowcolor{cyan!15} UNIP-S & 41.9 & \textbf{70.75} & \textbf{51.81} & \textbf{71.55} & \textbf{64.70} \\
        & & \plus{+1.42} & \plus{+4.66} & \plus{+1.75} & \plus{+2.61} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
  \end{minipage}
  \hfill
  \begin{minipage}{0.51\linewidth}
  \centering
    \caption{Comparison with other methods. All the compared results except PAD are borrowed from TINN. Training epochs of SODA and MFNet-T are 200 and 300.}
    \label{tab:sota_comparison}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{0.8mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c c}
        \toprule
        Methods & Params(M) & SODA & MFNet-T \\
        \midrule
        DeepLab V3+ \citep{deeplabv3+} & 62.7  & 68.73 & 49.80  \\
        PSPNet \citep{pspnet} & 68.1 & 68.68 & 45.24 \\
        UPerNet \citep{upernet} & 72.3 & 67.45 & 48.56 \\
        SegFormer \citep{segformer} & 84.7 & 67.86 & 50.68 \\
        ViT-Adapter \citep{vitadapter} & 99.8 & 68.12 & 50.62 \\
        Mask2Former \citep{mask2former} & 216.0 & 67.58 & 51.30 \\
        MaskDINO \citep{maskdino} & 223.0 & 66.32 & 51.03 \\
        \midrule
        EC-CNN \citep{soda} & 54.5 & 65.87 & 47.56 \\
        MCNet \citep{mcnet} & 35.7 & 63.89 & 43.15 \\
        PAD (MAE-B) \citep{pad} & 164.9 & 69.71 & 50.14 \\
        TINN \citep{tinn} & 85.3 & 69.45 & 51.93  \\
        \midrule
        \rowcolor{cyan!15} UNIP-T (MAE-L) & 11.0 & 67.29 & 50.39 \\
        \rowcolor{cyan!15} UNIP-S (MAE-L) & 41.9 & \underline{71.35} & \underline{53.76} \\
        \rowcolor{cyan!15} UNIP-B (MAE-L) & 163.7 & \textbf{72.19} & \textbf{54.35} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
  \end{minipage}
\end{table}

==> tab_tex/distill_setting.tex <==
\begin{table}[t]
    \caption{\textbf{Distillation setting.}}
    \label{tab:distill_setting}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{1.5mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c}
        \toprule
        Hyperparameters  &  Value \\
        \midrule
        Input resolution  &  224 $\times$  224 \\
        Training epochs &  100 \\
        Warmup epochs  &  5  \\
        Optimizer  &  AdamW  \\
        Base learning rate  & 1e-4  \\
        Weight decay  & 0.05  \\
        Optimizer momentum  &  $\beta_1, \beta_2=$ 0.9, 0.95 \\
        Batch size  &  4096 \\
        Learning rate schedule  &  Cosine decay  \\
        \bottomrule
    \end{tabular}}}
    \vspace{-2mm}
\end{table}

==> tab_tex/domain_gap.tex <==
\begin{table}[t]
    \centering
    \caption{The cosine similarity between pre-training and downstream datasets. The embeddings of images are extracted by DINO-Base. The similarity is averaged over all pairwise images from different datasets.}
    \label{tab:domain_gap}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.2mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c}
        \toprule
        \multirow{2}{*}{Pre-training dataset} & \multicolumn{3}{c}{Downstream dataset} \\
        \cmidrule(lr){2-4} 
        & SODA & MFNet-T & SCUT-Seg \\
        \midrule
        ImageNet-1K & 0.083 & 0.074 & 0.081 \\
        COCO & 0.111 & 0.101 & 0.106  \\
        Mixed dataset & 0.200 & 0.227 & 0.236 \\
        Mixed dataset (gray) & \textbf{0.216} & \textbf{0.246} & \textbf{0.254} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/fpn_ablation.tex <==
\begin{table}[t]
    \centering
    \caption{Ablations for different feature pyramid configurations. The student models are ViT-Small.}
    \label{tab:fpn_ablation}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.2mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c}
        \toprule
        Teacher & Last-Layer & SODA & MFNet-T & SCUT-Seg & Mean \\
        \midrule
        \multirow{2}{*}{MAE-L} & \xmark & 69.54 & 50.18 & 70.63 & 63.45 \\
        & \rowcolor{cyan!15} \cmark & \textbf{70.99} & \textbf{51.32} & \textbf{70.79} & \textbf{64.37} \\
        \midrule
        \multirow{2}{*}{DINO-B} & \xmark & 68.56 & 49.44 & 68.49 & 62.16 \\
        & \rowcolor{cyan!15} \cmark & \textbf{69.35} & \textbf{49.95} & \textbf{69.70} & \textbf{63.00} \\
        \midrule
        \multirow{2}{*}{iBOT-L} & \xmark & 70.03 & 50.30 & 69.64 & 63.32 \\
        & \rowcolor{cyan!15} \cmark & \textbf{70.75} & \textbf{51.81} & \textbf{71.55} & \textbf{64.70} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/layer_ablation.tex <==
\begin{table}[t]
    \centering
    \caption{Ablations for different target layers of distillation. The student models are ViT-Small.}
    \label{tab:layer_ablation}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.2mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c}
        \toprule
        Teacher & Layer & SODA & MFNet-T & SCUT-Seg & Mean \\
        \midrule
        \multirow{2}{*}{MAE-Large} & \rowcolor{gray!20} 18 & \textbf{70.99} & \textbf{51.32} & \textbf{70.79} & \textbf{64.37}  \\
        & 24 & 67.74 & 50.39 & 69.00 & 62.38  \\
        \midrule
        \multirow{2}{*}{DINO-Base} & \rowcolor{gray!20} 9 & \textbf{69.35} & \textbf{49.95} & \textbf{69.70} & \textbf{63.00}  \\
        & 12 & 68.50 & 48.40 & 69.67 & 62.19 \\
        \midrule
        \multirow{2}{*}{iBOT-Large} & 18 & 70.83 & 51.61 & 71.12 & 64.52 \\
        & \rowcolor{gray!20} 24 & \textbf{70.75} & \textbf{51.81} & \textbf{71.55} & \textbf{64.70} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/llp_base.tex <==
\begin{table}[t]
    \centering
    \caption{Caption}
    \label{tab:llp_base}
    \centering
    \setlength{\tabcolsep}{1.2mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c c c c c}
        \toprule
         \multirow{2}{*}{Methods} & \multicolumn{9}{c}{Layer (ViT-Base)}  \\
         \cmidrule(lr){2-10}
         & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
         \midrule
         MAE & 18.18 & 21.69 & 25.28 & 28.03 & 33.49 & 34.84 & 36.54 & \textbf{37.28} & 36.43 \\
         CrossMAE & 19.23 & 22.26 & 26.07 & 29.26 & 31.41 & 33.58 & 34.78 & 36.25 & \textbf{36.41} \\
         DeiT & 24.24 & 29.31 & 38.24 & 48.54 & 53.80 & 55.86 & \textbf{56.37} & 55.47 & 54.59 \\
         DeiT III & 29.82 & 41.16 & 51.14 & 55.48 & \textbf{57.18} & 56.70 & 55.51 & 54.90 & 54.89 \\
         DINO & 39.98 & 48.51 & 53.42 & 55.83 & 57.04 & \textbf{57.05} & 56.04 & 54.96 & 54.55 \\
         iBOT & 41.12 & 48.81 & 53.70 & 56.49 & 58.05 & \textbf{58.10} & 57.79 & 57.48 & 57.23 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/llp_large.tex <==
\begin{table}[t]
    \centering
    \caption{Caption}
    \label{tab:llp_large}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.0mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c c c c c c c c c c c c c c}
        \toprule
         \multirow{2}{*}{Methods} & \multicolumn{17}{c}{Layer (ViT-Large)}  \\
         \cmidrule(lr){2-18}
         & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 \\
         \midrule
         MAE & 27.50 & 33.39 & 38.50 & 40.05 & 41.10 & 42.79 & 45.25 & \textbf{47.06} & 46.85 & 46.88 & 46.48 & 46.52 & 46.11 & 45.94 & 45.08 & 44.05 & 42.23 \\
         DeiT & 36.75 & 42.54 & 48.14 & 51.79 & 54.82 & 56.57 & 57.33 & 57.84 & 58.01 & 58.05 & 58.12 & \textbf{58.22} & 57.83 & 57.81 & 57.46 & 57.12 & 57.17 \\
         iBOT & 51.38 & 55.07 & 57.81 & 59.01 & 60.65 & 61.62 & 62.18 & 62.53 & 62.48 & 62.42 & 62.63 & \textbf{62.75} & 62.64 & 62.60 & 62.60 & 62.49 & 62.44 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/llp_small.tex <==
\begin{table}[t]
    \centering
    \caption{Caption}
    \label{tab:llp_small}
    \centering
    \setlength{\tabcolsep}{1.2mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c c c c c}
        \toprule
         \multirow{2}{*}{Methods} & \multicolumn{9}{c}{Layer (ViT-Small)}  \\
         \cmidrule(lr){2-10}
         & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
         \midrule
         MAE & 16.95 & 19.48 & 21.60 & 25.11 & 27.98 & 29.98 & 30.67 & \textbf{31.24} & 30.39 \\
         CrossMAE & 16.07 & 17.02 & 19.15 & 22.64 & 27.10 & 29.32 & 31.09 & 31.23 & \textbf{31.98} \\
         DeiT & 21.84 & 25.78 & 31.79 & 37.57 & \textbf{38.31} & 38.07 & 36.39 & 34.89 & 34.67 \\
         DeiT III & 21.21 & 29.04 & 38.83 & 47.24 & \textbf{50.58} & 50.20 & 49.35 & 44.92 & 43.11 \\
         DINO & 27.60 & 35.60 & 44.18 & 49.81 & 53.42 & \textbf{53.49} & 51.50 & 48.23 & 47.43 \\
         iBOT & 31.15 & 38.34 & 44.64 & 50.86 & 53.09 & \textbf{54.96} & 54.60 & 53.64 & 53.33 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/pyramid.tex <==
\begin{table}[t]
    \centering
    \caption{The fine-tuning performance on SODA of different pyramid configurations. The pre-trained backbones are either frozen or unfrozen.}
    \label{tab:pyramid}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.2mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c}
        \toprule
        Methods & Configurations & Features & Frozen & Unfrozen  \\
        \midrule
        \multirow{3}{*}{MAE-Small} & \{4,6,8,12\} & - & - & 63.36 \\
        & \{9,9,9,9\} & low-level &  & 62.44 \\
        & \{12,12,12,12\} & mid-level & \textbf{52.26} & \textbf{64.39} \\
        \midrule
        \multirow{3}{*}{DINO-Small}  & \{4,6,8,12\} & - & - & 68.56 \\
        & \{9,9,9,9\} & mid-level & \textbf{62.45} & 68.13 \\
        & \{12,12,12,12\} & high-level & 61.01 & \textbf{68.72} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}



==> tab_tex/rgb_infrared.tex <==
\begin{table}[t]
    \caption{The FT performance on RGB and infrared semantic segmentation datasets.}
    \label{tab:rgb_infrared}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.0mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c}
        \toprule
        \multirow{2}{*}{Methods} & \multicolumn{2}{c}{RGB} & \multicolumn{3}{c}{Infrared} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-6}
        & ADE20K & MFNet-RGB & MFNet-T & SODA & SCUT-Seg \\
        \midrule
        DeiT-B & 47.4 & 57.07 & \textbf{48.59} & 69.73 & 69.35 \\
        DINO-B & 46.8 & 55.20 & 48.54 & \textbf{69.79} & \textbf{69.82} \\
        MAE-B & \textbf{48.1} & \textbf{57.29} & 46.78 & 68.18 & 67.86 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}



==> tab_tex/rgb_llp.tex <==
\begin{table}[t]
    \caption{The layerwise linear probing (LLP) performance on RGB and depth datasets. Training epochs are 30 for ADE20K and 100 for others.}
    \label{tab:rgb_llp}
    \vspace{1mm}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{0.8mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c c}
        \toprule
        \multirow{3}{*}{Modality} & \multirow{3}{*}{Dataset} & \multicolumn{2}{c}{DINO-S} & \multicolumn{2}{c}{DeiT-S} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6}
        & & Layer 9 & Layer 12  & Layer 9 & Layer 12 \\
        & & \textcolor{gray}{(\textit{Hybrid})} & \textcolor{gray}{(\textit{Global})} & \textcolor{gray}{(\textit{Hybrid})} & \textcolor{gray}{(\textit{Global})} \\
        \midrule
        \multirow{2}{*}{RGB} & ADE20K \citep{ade20k} & \textbf{26.11} & 23.15 & \textbf{24.35} & 22.68  \\
        & MFNet-RGB \citep{mfnet} & \textbf{38.94} & 37.53  & \textbf{30.43} & 29.44 \\
        \midrule
        \multirow{2}{*}{Depth} & NYUDepthv2 \citep{nyuv2} & \textbf{17.25} & 15.29 & \textbf{5.55} & 5.15 \\
        & SUN-RGBD \citep{sunrgbd} & \textbf{13.17} & 11.41 & \textbf{5.61} & 4.94 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-6mm}
\end{table}

==> tab_tex/sota_comparison.tex <==
\begin{table}[t]
    \centering
    \caption{Comparison with other methods (FT). All the compared results except PAD are borrowed from TINN. Training epochs of SODA and MFNet-T are 200 and 300.}
    \label{tab:sota_comparison}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{0.8mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c c c}
        \toprule
        Methods & Params(M) & SODA & MFNet-T \\
        \midrule
        DeepLab V3+ \citep{deeplabv3+} & 62.7  & 68.73 & 49.80  \\
        PSPNet \citep{pspnet} & 68.1 & 68.68 & 45.24 \\
        UPerNet \citep{upernet} & 72.3 & 67.45 & 48.56 \\
        SegFormer \citep{segformer} & 84.7 & 67.86 & 50.68 \\
        ViT-Adapter \citep{vitadapter} & 99.8 & 68.12 & 50.62 \\
        Mask2Former \citep{mask2former} & 216.0 & 67.58 & 51.30 \\
        MaskDINO \citep{maskdino} & 223.0 & 66.32 & 51.03 \\
        \midrule
        EC-CNN \citep{soda} & 54.5 & 65.87 & 47.56 \\
        MCNet \citep{mcnet} & 35.7 & 63.89 & 43.15 \\
        PAD (MAE-B) \citep{pad} & 164.9 & 69.71 & 50.14 \\
        TINN \citep{tinn} & 85.3 & 69.45 & 51.93  \\
        \midrule
        \rowcolor{cyan!15} UNIP-T (MAE-L) & 11.0 & 67.29 & 50.39 \\
        \rowcolor{cyan!15} UNIP-S (MAE-L) & 41.9 & \underline{71.35} & \underline{53.76} \\
        \rowcolor{cyan!15} UNIP-B (MAE-L) & 163.7 & \textbf{72.19} & \textbf{54.35} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/topk.tex <==
\begin{table}[t]
    \caption{The FT performance of using multiple layers of the teacher model for distillation. The teacher and student models are MAE-L and UNIP-S.}
    \label{tab:topk}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.0mm}{
    \scalebox{1.0}{
    \begin{tabular}{l c c c c}
        \toprule
        Layer & SODA & MFNet-T & SCUT-Seg & Mean \\
        \midrule
        \rowcolor{cyan!15} 18 & \textbf{70.99} & \textbf{51.32} & \textbf{70.79} & \textbf{64.37} \\
        17+18 & 69.59 & 51.33 & 69.47 & 63.46 \\
        17+18+19 & 69.13 & 49.96 & 67.73 & 62.27 \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}

==> tab_tex/wo_pretrain.tex <==
\begin{table}[t]
    \centering
    \caption{Comparison of pre-training.}
    \label{tab:wo_pretrain}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.2mm}{
    \scalebox{1.0}{
    \begin{tabular}{c c c c c}
        \toprule
        Pre-training & Tiny & Small & Base & Large \\
        \midrule
        \xmark & 30.64 & 36.82 & 39.14 & 39.31  \\
        \cmark & \textbf{51.53} & \textbf{59.65} & \textbf{62.53} & \textbf{64.34}
        \\
        & \textcolor{red}{+20.89} & \textcolor{red}{+22.83} & \textcolor{red}{+23.39} & \textcolor{red}{+25.03} \\
        \bottomrule
    \end{tabular}}}
    \vspace{-4mm}
\end{table}
